MobileRec: A Large-Scale Dataset for Mobile Apps Recommendation

Recommender systems have become ubiquitous in our digital lives, from recommending products on e-commerce websites to suggesting movies and music on streaming platforms. Existing recommendation datasets, such as Amazon Product Reviews and MovieLens, greatly facilitated the research and development of recommender systems in their respective domains. While the number of mobile users and applications (aka apps) has increased exponentially over the past decade, research in mobile app recommender systems has been significantly constrained, primarily due to the lack of high-quality benchmark datasets, as opposed to recommendations for products, movies, and news. To facilitate research for app recommendation systems, we introduce a large-scale dataset, called MobileRec. We constructed MobileRec from users' activity on the Google play store. MobileRec contains 19.3 million user interactions (i.e., user reviews on apps) with over 10K unique apps across 48 categories. MobileRec records the sequential activity of a total of 0.7 million distinct users. Each of these users has interacted with no fewer than five distinct apps, which stands in contrast to previous datasets on mobile apps that recorded only a single interaction per user. Furthermore, MobileRec presents users' ratings as well as sentiments on installed apps, and each app contains rich metadata such as app name, category, description, and overall rating, among others. We demonstrate that MobileRec can serve as an excellent testbed for app recommendation through a comparative study of several state-of-the-art recommendation approaches. The quantitative results can act as a baseline for other researchers to compare their results against. The MobileRec dataset is available at https://huggingface.co/datasets/recmeapp/mobilerec.

==> tables/tbl_bl_results_old.tex <==
\begin{table*}[t]
\par\vspace{20pt}\par
\resizebox{\textwidth}{!}{%

}
\end{table*}

==> tables/tbl_statistics_v0.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%

\begin{tabular}{cllllllll}
\toprule
\textbf{Datasets}                      & \textbf{Users with \textgreater 4 interactions} & \textbf{Items with \textgreater 19 interactions} & \textbf{Max. interactions from a user} & \textbf{Min. interactions from a user} & \textbf{Avg. \# items interacted by a user} & \textbf{Max. interactions on an item} & \textbf{Min. interactions on an item} & \textbf{Avg. interactions per item} \\ \hline
\multicolumn{1}{c|}{\textbf{Beauty}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{ML-1M}}    & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Yelp}}     & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Stream}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{ML-20M}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Sports}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{LastFM}}   & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Toys}}     & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Games}}    & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\
\multicolumn{1}{c|}{\textbf{Clothing}} & \multicolumn{1}{l|}{}                           & \multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                  & \multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}                 &                                     \\ \hline
\textbf{GooglePlay (Ours)}             &                                                 &                                                  &                                        &                                        &                                             &                                       &                                       &           \\    
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tbl_statistics_v1.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcllllllllll}
\toprule
\multicolumn{1}{c}{\textbf{Datasets}}                                 & \textbf{Beauty} & \multicolumn{1}{c}{\textbf{ML-1M}} & \multicolumn{1}{c}{\textbf{Yelp}} & \multicolumn{1}{c}{\textbf{Stream}} & \multicolumn{1}{c}{\textbf{ML-20M}} & \multicolumn{1}{c}{\textbf{Sports}} & \textbf{LastFM} & \multicolumn{1}{c}{\textbf{Toys}} & \multicolumn{1}{c}{\textbf{Games}} & \multicolumn{1}{c}{\textbf{Clothing}} & \multicolumn{1}{c}{\textbf{MobileRec (Ours)}} \\ \hline
\multicolumn{1}{l|}{\textbf{Total interactions}}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{19297020}}                                          \\
\multicolumn{1}{l|}{\textbf{Users with \textgreater 4 interactions}}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{700111}}                                          \\
\multicolumn{1}{l|}{\textbf{Items with \textgreater 14 interactions}} & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &                 \multicolumn{1}{c}{\textbf{10173}}                               \\
\multicolumn{1}{l|}{\textbf{Max. interactions from a user}}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &        \multicolumn{1}{c}{\textbf{256}}                                        \\
\multicolumn{1}{l|}{\textbf{Min. interactions from a user}}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &      \multicolumn{1}{c}{\textbf{5}}                                          \\
\multicolumn{1}{l|}{\textbf{Avg. interactions by a user}}      & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &             \multicolumn{1}{c}{\textbf{27.5628}}                                   \\
\multicolumn{1}{l|}{\textbf{Max. interactions on an item}}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &                    \multicolumn{1}{c}{\textbf{14345}}                            \\
\multicolumn{1}{l|}{\textbf{Min. interactions on an item}}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &            \multicolumn{1}{c}{\textbf{20}}                                    \\
\multicolumn{1}{l|}{\textbf{Avg. interactions per item}}              & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    & \multicolumn{1}{l|}{}                 &     \multicolumn{1}{c}{\textbf{1896.8858}}    \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/tbl_statistics_v2.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|clllllllll|l}
\toprule
\multicolumn{1}{c|}{\textbf{Datasets}}           & \textbf{Beauty} & \multicolumn{1}{c}{\textbf{ML-1M}} & \multicolumn{1}{c}{\textbf{Yelp}} & \multicolumn{1}{c}{\textbf{Stream}} & \multicolumn{1}{c}{\textbf{ML-20M}} & \multicolumn{1}{c}{\textbf{Sports}} & \textbf{LastFM} & \multicolumn{1}{c}{\textbf{Toys}} & \multicolumn{1}{c}{\textbf{Games}} & \multicolumn{1}{c|}{\textbf{Clothing}} & \multicolumn{1}{c}{\textbf{GooglePlay (Ours)}} \\ \hline
\textbf{Users with \textgreater 4 interactions}  & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Items with \textgreater 19 interactions} & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Max. interactions from a user}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Min. interactions from a user}           & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Avg. \# items interacted by a user}      & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Max. interactions on an item}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Min. interactions on an item}            & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\textbf{Avg. interactions per item}              & \textbf{}       &                                    &                                   &                                     &                                     &                                     &                 &                                   &                                    &                                        &                                                \\ \hline
\\
\bottomrule
\end{tabular}
}
\end{table*}
